Beyond Linear Approximations: A Novel Pruning Approach for Attention Matrix

Large Language Models (LLMs) have shown immense potential in enhancing various aspects of our daily lives, from conversational AI to search and AI assistants. However, their growing capabilities come at the cost of extremely large model sizes, making deployment on edge devices challenging due to memory and computational constraints. This paper introduces a novel approach to LLM weight pruning that directly optimizes for approximating the attention matrix, a core component of transformer architectures. Unlike existing methods that focus on linear approximations, our approach accounts for the non-linear nature of the Softmax attention mechanism. We provide theoretical guarantees for the convergence of our Gradient Descent-based optimization method to a near-optimal pruning mask solution. Our empirical results demonstrate the effectiveness of our non-linear pruning approach in maintaining model performance while significantly reducing computational costs, which is beyond the current state-of-the-art methods, i.e., SparseGPT and Wanda, by a large margin. This work establishes a new theoretical foundation for pruning algorithm design in LLMs, potentially paving the way for more efficient LLM inference on resource-constrained devices.

==> 10_app_attention_prune.tex <==
\section{Definitions of optimal pruning mask}\label{sec:app:pruning}


We aim to determine the optimal pruning mask $M$ for the attention weights, ensuring that the pruned attention matrix remains sufficiently close to the original attention matrix.

We provide the formal definition for the causal attention mask. 

\begin{definition}[Causal attention mask, \cite{lls+24_conv}]\label{def:mask}
    We define the causal attention mask as $M_c \in \{0,1\}^{n\times n}$, where $(M_c)_{i,j} = 1$ if $i \ge j$ and $(M_c)_{i,j} = 0$ otherwise.
\end{definition}

\begin{definition}[Attention Weights Pruning]
If the following conditions hold:
\begin{itemize}
\item Let $M \in [0,1]^{d \times d}$ be the pruning mask.
\item Let $X \in \R^{n \times d}, W \in \R^{d \times d}$.
\item Let $M_c \in \{0,1\}^{n\times n}$ be the causal attention mask defined in Definition~\ref{def:mask}. 
\item Let $A := \exp(XWX^\top)\circ M_c$ and $\wt{A} := \exp(X(M \circ W)X^\top)\circ M_c$.
\item Let $D := \diag(A \cdot {\bf 1}_n)$ and $\wt{D} := \diag(\wt{A} \cdot {\bf 1}_n)$.
\item Let $\lambda \in \R_+$ be the regularization parameter.
\end{itemize}



Then, we define the Attention Weights Pruning problem to be
\begin{align*}
    \min_M ~ \frac{1}{2} \|D^{-1} A -  \wt{D}^{-1} \wt{A}\|_F^2 + \frac{1}{2} \lambda \|M\|_F^2
\end{align*}
\end{definition}



We now define the loss function we are concerned about.
\begin{definition}[Loss Function]
If the following conditions hold:
\begin{itemize}
    \item Let $X \in \R^{n \times d}, W \in \R^{d \times d}, M \in [0,1]^{d \times d}, \lambda \in \R_+$.
    \item Let $M_c \in \{0,1\}^{n\times n}$ be the causal attention mask defined in Definition~\ref{def:mask}.
    \item Let $A := \exp(XWX^\top)\circ M_c$ and $\wt{A} := \exp(X(M \circ W)X^\top)\circ M_c$.
    \item Let $D := \diag(A \cdot {\bf 1}_n)$ and $\wt{D} := \diag(\wt{A} \cdot {\bf 1}_n)$.
    \item Let $\lambda \in \R_+$ be the regularization parameter.
\end{itemize}

We define the loss function to be
\begin{align*}
    \mathcal{L}(M) := \frac{1}{2} \|D^{-1} A -  \wt{D}^{-1} \wt{A}\|_F^2 + \frac{1}{2} \lambda \|M\|_F^2
\end{align*}
\end{definition}

